Zero-shot Cross-lingual Transfer is Under-specified Optimization

Pretrained multilingual encoders enable zero-shot cross-lingual transfer, but often produce unreliable models that exhibit high performance variance on the target language. We postulate that this high variance results from zero-shot cross-lingual transfer solving an under-specified optimization problem. We show that any linear-interpolated model between the source language monolingual model and source + target bilingual model has equally low source language generalization error, yet the target language generalization error reduces smoothly and linearly as we move from the monolingual to bilingual model, suggesting that the model struggles to identify good solutions for both source and target languages using the source language alone. Additionally, we show that zero-shot solution lies in non-flat region of target language error generalization surface, causing the high variance.

==> Zero-shot Cross-lingual Transfer is Under-specified Optimization_arXiv/analogy.tex <==
\section{Cross-task and -language Analogy}


\input{result/reference}

\input{result/analogy-shift}

In \cref{sec:analysis}, we show that the zero-shot cross-lingual transfer is an under-specified optimization problem. \textit{Can we search the parameter space without access to the target language data?} \citet{mikolov2013distributed} show that there exist linear arithmetic in the embedding space, for example $v(\texttt{queen}) \approx v(\texttt{women}) + v(\texttt{king}) - v(\texttt{men})$.
Assuming we have both language supervision for a reference task, it inspires the setup shown by \cref{tab:reference}.
The goal is to figure out model \D~using the three models \A, \B, and \C.
Similar to the linear arithmetic in word embeddings, linear analogy assumes that the shift (of encoder) between monolingual and bilingual models of different tasks are similar. Specifically, $\mathcal{D} \approx \mathcal{C} + \mathcal{B} - \mathcal{A}$. Note we only modify the encoder, and we reuse the task-specific layer from \C.



\paragraph{Experiment} Similar to \cref{sec:analysis}, we consider the same eight target languages and English as the source language. We select the same four tasks as both the task of interest and reference task.
We report the average of three runs, each with a model trained with a different random seed. To aggregate the result, we averaged over the non-English performance.

\paragraph{Findings} \cref{tab:main} shows a mixed analogy result. We observe that XNLI is not an ideal reference task, as it leads to a significant performance drop. An possible reason might be that the task is drastically different from other token-level tasks. The most notable performance boost setups are POS and Parsing as reference tasks and task of interest and vice versa. One underlying reason could be that both tasks have the same underlying text, as they belong to the same treebank. It points to a new setup: automatically labelling an existing English dataset of task of interest and target language corpus with simpler tasks (e.g. NER or POS) and existing system, and creating ``Silver'' reference tasks. We will leave it as future work.



==> Zero-shot Cross-lingual Transfer is Under-specified Optimization_arXiv/result/dataset-stats.tex <==
\begin{table}[h]
\begin{center}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}[b]{lccc}
\toprule
 & \multirow{2}{*}{XNLI} & \multirow{2}{*}{NER} & POS tagging \\
 & & & Parsing\\
\midrule
en-train & 392703 & 20000 & 12543 \\
en-dev & 2490 & 10000 & 2002 \\
\midrule
ar-train & 392703 & 20000 & 6075 \\
ar-dev & 2490 & 10000 & 909 \\
\midrule
de-train & 392703 & 20000 & 13814 \\
de-dev & 2490 & 10000 & 799 \\
\midrule
es-train & 392703 & 20000 & 14187 \\
es-dev & 2490 & 10000 & 1400 \\
\midrule
fr-train & 392703 & 20000 & 14449 \\
fr-dev & 2490 & 10000 & 1476 \\
\midrule
hi-train & 392703 & 5000 & 13304 \\
hi-dev & 2490 & 1000 & 1659 \\
\midrule
ru-train & 392703 & 20000 & 3850 \\
ru-dev & 2490 & 10000 & 579 \\
\midrule
vi-train & 392703 & 20000 & 1400 \\
vi-dev & 2490 & 10000 & 800 \\
\midrule
zh-train & 392703 & 20000 & 3997 \\
zh-dev & 2490 & 10000 & 500 \\
\bottomrule
\end{tabular}
}
\caption{Number of examples.\label{tab:stat}}
\end{center}
\end{table}

==> analogy.tex <==
\section{Cross-task and -language Analogy}


\input{result/reference}

\input{result/analogy-shift}

In \cref{sec:analysis}, we show that the zero-shot cross-lingual transfer is an under-specified optimization problem. \textit{Can we search the parameter space without access to the target language data?} \citet{mikolov2013distributed} show that there exist linear arithmetic in the embedding space, for example $v(\texttt{queen}) \approx v(\texttt{women}) + v(\texttt{king}) - v(\texttt{men})$.
Assuming we have both language supervision for a reference task, it inspires the setup shown by \cref{tab:reference}.
The goal is to figure out model \D~using the three models \A, \B, and \C.
Similar to the linear arithmetic in word embeddings, linear analogy assumes that the shift (of encoder) between monolingual and bilingual models of different tasks are similar. Specifically, $\mathcal{D} \approx \mathcal{C} + \mathcal{B} - \mathcal{A}$. Note we only modify the encoder, and we reuse the task-specific layer from \C.



\paragraph{Experiment} Similar to \cref{sec:analysis}, we consider the same eight target languages and English as the source language. We select the same four tasks as both the task of interest and reference task.
We report the average of three runs, each with a model trained with a different random seed. To aggregate the result, we averaged over the non-English performance.

\paragraph{Findings} \cref{tab:main} shows a mixed analogy result. We observe that XNLI is not an ideal reference task, as it leads to a significant performance drop. An possible reason might be that the task is drastically different from other token-level tasks. The most notable performance boost setups are POS and Parsing as reference tasks and task of interest and vice versa. One underlying reason could be that both tasks have the same underlying text, as they belong to the same treebank. It points to a new setup: automatically labelling an existing English dataset of task of interest and target language corpus with simpler tasks (e.g. NER or POS) and existing system, and creating ``Silver'' reference tasks. We will leave it as future work.


